What Types of Questions Require Conversation to Answer? A Case Study of AskReddit Questions

The proliferation of automated conversational systems such as chatbots, spoken-dialogue systems, and smart speakers, has significantly impacted modern digital life. However, these systems are primarily designed to provide answers to well-defined questions rather than to support users in exploring complex, ill-defined questions. In this paper, we aim to push the boundaries of conversational systems by examining the types of nebulous, open-ended questions that can best be answered through conversation. We first sampled 500 questions from one million open-ended requests posted on AskReddit, and then recruited online crowd workers to answer eight inquiries about these questions. We also performed open coding to categorize the questions into 27 different domains. We found that the issues people believe require conversation to resolve satisfactorily are highly social and personal. Our work provides insights into how future research could be geared to align with users' needs.

==> table/allcategories.tex <==
\begin{table*}[h]
    \centering \small
    \begin{tabular}{lrl}
        \toprule
        \multicolumn{1}{c}{\textbf{Category}} & \multicolumn{1}{c}{\textbf{\# Questions}} & \multicolumn{1}{c}{\textbf{Brief Description}} \\ \midrule
        science                           & 13  & Science  \\
        history\_old\_days\_future        & 12  & History and discussion about the past or future \\
        career                            & 11  & Career  \\
        food                              & 10  & Food \\
        human\_body                        & 10  & Human body mechanism and functions\\
        legal\_regulation                  & 10  & Law, legal questions, general regulations\\
        news\_events                       & 9   & News and real-life events\\
        social\_etiquette                  & 9   & Social etiquette\\
        mental\_health                     & 8   & Mental health\\
        learning\_skills                   & 7   & Learning and acquire skills\\
        personal\_finance                  & 7   & Personal finance\\
        worldwide\_society\_effect\_impact & 7   & Worldwide scale discussion/societal changes and impact\\
        NSFW\_sensitive                    & 6   & Not safe for work; not suitable for work and sensitive topics\\
        politics                          & 6   & Politics\\
        relationship                      & 6   & Couple relationships\\
        religion                          & 5   & Religion\\
        Others                            & 45  & Categories that appear fewer than five times \\
        \bottomrule
        \end{tabular}
    \caption{The 17 lowest-scoring categories. (See Table~\ref{tab:category} for the top 10 categories.)}
    \label{tab:category-rest}
\end{table*}

==> table/category-correlation-ask-for-help.tex <==
\begin{table}[t]
\small \centering
    \begin{tabular}{lrlr}
    \toprule
    \multicolumn{1}{c}{\textbf{Category}} & \textbf{Ask-for-Help} & \multicolumn{1}{c}{\textbf{Category}} & \textbf{Ask-for-Help} \\ \midrule
    \textbf{religion} & -0.757 & \textbf{history\_old\_days\_future} & 0.311 \\
    \textbf{personal\_finance} & -0.380 & \textbf{reddit\_tech} & 0.392 \\
    \textbf{NSFW\_sensitive} & -0.166 & \textbf{culture\_believe\_language} & 0.403 \\
    \textbf{career} & -0.062 & \textbf{dailylife\_hack\_for\_fun\_home} & 0.429 \\
    \textbf{politics} & -0.049 & \textbf{news\_events} & 0.451 \\
    \textbf{mental\_health} & 0.092 & \textbf{others} & 0.462 \\
    \textbf{food} & 0.101 & \textbf{medical\_health\_diet} & 0.524 \\
    \textbf{movie\_music\_media\_hobby\_sport} & 0.179 & \textbf{legal\_regulation} & 0.538 \\
    \textbf{relationship} & 0.242 & \textbf{help\_find\_things} & 0.549 \\
    \textbf{social\_etiquette} & 0.268 & \textbf{science} & 0.584 \\
    \textbf{worldwide\_society\_effect\_impact} & 0.279 & \textbf{tech} & 0.621 \\
    \textbf{country\_location\_travel} & 0.283 & \textbf{socializing} & 0.719 \\
    \textbf{life\_suggestion} & 0.291 & \textbf{human\_body} & 0.792 \\
     & \multicolumn{1}{l}{} & \textbf{learning\_skills} & 0.908 \\ 
     \bottomrule
    \end{tabular}
    \caption{Correlation between Ask-for-Help and Conversation in different categories. We hypothesized the negative correlations were caused by people not willing to disclose their identity.}
    \label{tab:category-correlation-ask-for-help}
\end{table}
